Nucleus I: Adjunction spectra in recommender systems and descent

Recommender systems build user profiles using concept analysis of usage matrices. The concepts are mined as spectra and form Galois connections. Descent is a general method for spectral decomposition in algebraic geometry and topology which also leads to generalized Galois connections. Both recommender systems and descent theory are vast research areas, separated by a technical gap so large that trying to establish a link would seem foolish. Yet a formal link emerged, all on its own, bottom-up, against authors' intentions and better judgment. Familiar problems of data analysis led to a novel solution in category theory. The present paper arose from a series of earlier efforts to provide a top-down account of these developments.

==> PIC/trust-FCA-decomp.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Thu Apr 09 09:43:49 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="10" x-max="110" y-min="-2.5" y-max="130" auto-bounding="true">
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(22,91);(22,91);(45,45.62);(45,45.62)"
%	 stroke-overstrike= "true"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 />
%<parallelogram fill-color= "#0000ff"
%	 fill-style= "solid"
%	 p3= "(102,67)"
%	 p2= "(102,63)"
%	 p1= "(98,63)"
%	 stroke-color= "#0000ff"
%	 />
%<ellipse fill-color= "#ff6666"
%	 fill-style= "solid"
%	 p3= "(21.5,57)"
%	 p2= "(21.5,53)"
%	 p1= "(18.5,53)"
%	 stroke-color= "#ff6666"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<parallelogram fill-color= "#0000ff"
%	 fill-style= "solid"
%	 p3= "(102,47)"
%	 p2= "(102,43)"
%	 p1= "(98,43)"
%	 stroke-color= "#0000ff"
%	 />
%<parallelogram fill-color= "#0000ff"
%	 fill-style= "solid"
%	 p3= "(102,87)"
%	 p2= "(102,83)"
%	 p1= "(98,83)"
%	 stroke-color= "#0000ff"
%	 />
%<ellipse fill-color= "#ff6666"
%	 fill-style= "solid"
%	 p3= "(21.5,77)"
%	 p2= "(21.5,73)"
%	 p1= "(18.5,73)"
%	 stroke-color= "#ff6666"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(32.5,98.75);(32.5,98.75);(43.75,100);(43.75,100)"
%	 stroke-overstrike= "true"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(70,74.38);(70,74.38);(96.25,66.25);(96.25,66.25)"
%	 arrow-head-width-minimum= "1.45"
%	 />
%<ellipse fill-color= "#ff6666"
%	 fill-style= "solid"
%	 p3= "(21.5,97)"
%	 p2= "(21.5,93)"
%	 p1= "(18.5,93)"
%	 stroke-color= "#ff6666"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<ellipse fill-color= "#ff6666"
%	 fill-style= "solid"
%	 p3= "(21.5,37)"
%	 p2= "(21.5,33)"
%	 p1= "(18.5,33)"
%	 stroke-color= "#ff6666"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(68.75,71.88);(68.75,71.88);(96.88,46.25);(96.88,46.25)"
%	 stroke-overstrike= "true"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(66.88,15);(66.88,15);(71.88,21.25);(71.88,21.25)"
%	 stroke-overstrike= "true"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(23.12,56.88);(23.12,56.88);(60.62,73.75);(60.62,73.75)"
%	 stroke-overstrike= "true"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(50.62,46.25);(50.62,46.25);(96.25,65);(96.25,65)"
%	 stroke-overstrike= "true"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(23.75,75.62);(23.75,75.62);(60,76);(60,76)"
%	 stroke-overstrike= "true"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.85"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(52.5,43.12);(52.5,43.12);(96.25,43.75);(96.25,43.75)"
%	 stroke-overstrike= "true"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(23.12,36.88);(23.12,36.88);(61.88,71.25);(61.88,71.25)"
%	 stroke-overstrike= "true"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(55.62,100.62);(55.62,100.62);(65,96.88);(65,96.88)"
%	 stroke-overstrike= "true"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,95)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ha$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hb$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hc$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hd$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(110,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hI$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(110,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hII$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(110,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hIII$
%</text>
%<parallelogram fill-color= "#0000ff"
%	 fill-style= "solid"
%	 p3= "(102,27)"
%	 p2= "(102,23)"
%	 p1= "(98,23)"
%	 stroke-color= "#0000ff"
%	 />
%<ellipse fill-color= "#ff6666"
%	 fill-style= "solid"
%	 p3= "(21.5,17)"
%	 p2= "(21.5,13)"
%	 p1= "(18.5,13)"
%	 stroke-color= "#ff6666"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(50.62,40);(50.62,40);(96.25,25);(96.25,25)"
%	 stroke-overstrike= "true"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(10,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\he$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(110,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hIV$
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(100,115)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\trustees
%</text>
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(20,115)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\trustors
%</text>
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(23,94);(23,94);(62,78);(62,78)"
%	 stroke-overstrike= "true"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(49.38,10.62);(49.38,10.62);(58.75,9.38);(58.75,9.38)"
%	 stroke-overstrike= "true"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(23.12,15.62);(23.12,15.62);(44.38,39.38);(44.38,39.38)"
%	 stroke-overstrike= "true"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 />
%<parallelogram fill-style= "solid"
%	 stroke-width= "0.55"
%	 p3= "(48.9,103.78)"
%	 p2= "(45.7,100.12)"
%	 p1= "(48.6,96.22)"
%	 />
%<parallelogram fill-style= "solid"
%	 stroke-width= "0.55"
%	 p3= "(65.15,78.78)"
%	 p2= "(61.95,75.12)"
%	 p1= "(64.85,71.22)"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(69.38,77.5);(69.38,77.5);(96.25,84.38);(96.25,84.38)"
%	 arrow-head-width-minimum= "1.45"
%	 />
%<parallelogram fill-style= "solid"
%	 stroke-width= "0.55"
%	 p3= "(47.65,46.9)"
%	 p2= "(44.45,43.24)"
%	 p1= "(47.35,39.35)"
%	 />
%<parallelogram fill-style= "solid"
%	 stroke-width= "0.55"
%	 p3= "(64.53,15.03)"
%	 p2= "(61.32,11.37)"
%	 p1= "(64.22,7.47)"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(50,15.62);(50,15.62);(58.75,11.25);(58.75,11.25)"
%	 stroke-overstrike= "true"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(51.25,20);(51.25,20);(59.38,13.12);(59.38,13.12)"
%	 stroke-overstrike= "true"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(53.75,23.75);(53.75,23.75);(60.62,15.62);(60.62,15.62)"
%	 stroke-overstrike= "true"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(57.5,25);(57.5,25);(62.5,16.25);(62.5,16.25)"
%	 stroke-overstrike= "true"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(68.12,13.12);(68.12,13.12);(75,18.75);(75,18.75)"
%	 stroke-overstrike= "true"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(54.38,98.75);(54.38,98.75);(62.5,92.5);(62.5,92.5)"
%	 stroke-overstrike= "true"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(51.88,96.88);(51.88,96.88);(58.75,89.38);(58.75,89.38)"
%	 stroke-overstrike= "true"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 />
%<multicurve arrow-head-length-scale= "1.55"
%	 arrow-global-scale-length= "1.45"
%	 fill-style= "none"
%	 right-arrow= "head"
%	 points= "(50,95);(50,95);(55,87.5);(55,87.5)"
%	 stroke-overstrike= "true"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 />
%<text fill-style= "none"
%	 text-vert-align= "center-v"
%	 anchor-point= "(55,112.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\concepts
%</text>
%<ellipse fill-style= "none"
%	 stroke-width= "0.5"
%	 p3= "(87.5,0)"
%	 p2= "(77.5,130)"
%	 p1= "(27.5,127.5)"
%	 stroke-color= "#990099"
%	 closure= "open"
%	 angle-end= "0"
%	 angle-start= "0"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(110,130)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(22,91)(45,45.62)
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,63)(102,63)(102,67)(98,67)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,55){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,43)(102,43)(102,47)(98,47)
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,83)(102,83)(102,87)(98,87)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,75){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(32.5,98.75)(43.75,100)
\psline[arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(70,74.38)(96.25,66.25)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,95){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,35){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(68.75,71.88)(96.88,46.25)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(66.88,15)(71.88,21.25)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,56.88)(60.62,73.75)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(50.62,46.25)(96.25,65)
\psline[border=0.85,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.75,75.62)(60,76)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(52.5,43.12)(96.25,43.75)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,36.88)(61.88,71.25)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(55.62,100.62)(65,96.88)
\rput(10,95){$\ha$}
\rput(10,75){$\hb$}
\rput(10,55){$\hc$}
\rput(10,35){$\hd$}
\rput(110,85){$\hI$}
\rput(110,65){$\hII$}
\rput(110,45){$\hIII$}
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,23)(102,23)(102,27)(98,27)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,15){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(50.62,40)(96.25,25)
\rput(10,15){$\he$}
\rput(110,25){$\hIV$}
\rput(100,115){\trustees}
\rput(20,115){\trustors}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23,94)(62,78)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(49.38,10.62)(58.75,9.38)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,15.62)(44.38,39.38)
\pspolygon[linewidth=0.55,fillstyle=solid](48.6,96.22)(45.7,100.12)(48.9,103.78)(51.8,99.88)
\pspolygon[linewidth=0.55,fillstyle=solid](64.85,71.22)(61.95,75.12)(65.15,78.78)(68.05,74.88)
\psline[arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(69.38,77.5)(96.25,84.38)
\pspolygon[linewidth=0.55,fillstyle=solid](47.35,39.35)(44.45,43.24)(47.65,46.9)(50.55,43.01)
\pspolygon[linewidth=0.55,fillstyle=solid](64.22,7.47)(61.32,11.37)(64.53,15.03)(67.43,11.13)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(50,15.62)(58.75,11.25)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(51.25,20)(59.38,13.12)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(53.75,23.75)(60.62,15.62)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(57.5,25)(62.5,16.25)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(68.12,13.12)(75,18.75)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(54.38,98.75)(62.5,92.5)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(51.88,96.88)(58.75,89.38)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(50,95)(55,87.5)
\rput(55,112.5){\concepts}
\newrgbcolor{userLineColour}{0.6 0 0.6}
\rput{94.66}(57.5,63.75){\psellipse[linewidth=0.5,linecolor=userLineColour](0,0)(65.2,-25.02)}
\end{pspicture}


==> PIC/trust-net-1.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Apr 08 23:23:57 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="10" x-max="110" y-min="3" y-max="105" auto-bounding="true">
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(22,81);(22,81);(96,14);(96,14)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<parallelogram p3= "(102,57)"
%	 fill-style= "solid"
%	 p2= "(102,53)"
%	 fill-color= "#0000ff"
%	 p1= "(98,53)"
%	 stroke-color= "#0000ff"
%	 />
%<ellipse p3= "(21.5,47)"
%	 fill-style= "solid"
%	 p2= "(21.5,43)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,43)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<parallelogram p3= "(102,37)"
%	 fill-style= "solid"
%	 p2= "(102,33)"
%	 fill-color= "#0000ff"
%	 p1= "(98,33)"
%	 stroke-color= "#0000ff"
%	 />
%<parallelogram p3= "(102,77)"
%	 fill-style= "solid"
%	 p2= "(102,73)"
%	 fill-color= "#0000ff"
%	 p1= "(98,73)"
%	 stroke-color= "#0000ff"
%	 />
%<ellipse p3= "(21.5,67)"
%	 fill-style= "solid"
%	 p2= "(21.5,63)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,63)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,85.62);(23.12,85.62);(95.62,76.88);(95.62,76.88)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 points= "(23.12,64.38);(23.12,64.38);(96.25,56.25);(96.25,56.25)"
%	 arrow-head-width-minimum= "1.45"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "0.2"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "1.1"
%	 points= "(23.12,62.5);(23.12,62.5);(96.25,36.88);(96.25,36.88)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "0.2"
%	 right-arrow= "head"
%	 />
%<ellipse p3= "(21.5,87)"
%	 fill-style= "solid"
%	 p2= "(21.5,83)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,83)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(21.5,27)"
%	 fill-style= "solid"
%	 p2= "(21.5,23)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,23)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23,82);(23,82);(95,40);(95,40)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(22.5,6.88);(22.5,6.88);(96.88,51.88);(96.88,51.88)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "0.2"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,46.88);(23.12,46.88);(96.25,73.12);(96.25,73.12)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "0.2"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.38,45.12);(23.38,45.12);(96.25,55);(96.25,55)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "0.2"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.85"
%	 points= "(23.75,65.62);(23.75,65.62);(96.62,74.38);(96.62,74.38)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "0.2"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,23.75);(23.12,23.75);(96.25,33.75);(96.25,33.75)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "0.2"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,26.88);(23.12,26.88);(96.88,71.25);(96.88,71.25)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "0.2"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.38,25.12);(23.38,25.12);(96.25,53.75);(96.25,53.75)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "0.2"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ha$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hb$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hc$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hI$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hII$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hIII$
%</text>
%<parallelogram p3= "(102,17)"
%	 fill-style= "solid"
%	 p2= "(102,13)"
%	 fill-color= "#0000ff"
%	 p1= "(98,13)"
%	 stroke-color= "#0000ff"
%	 />
%<ellipse p3= "(21.5,7)"
%	 fill-style= "solid"
%	 p2= "(21.5,3)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,3)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,3.75);(23.12,3.75);(96.88,13.75);(96.88,13.75)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "0.2"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\he$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hIV$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\trustees
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\trustors
%</text>
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23,84);(23,84);(96.25,57.5);(96.25,57.5)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,43.75);(23.12,43.75);(96.26,35.63);(96.26,35.63)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "0.2"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,5.62);(23.12,5.62);(96.88,32.5);(96.88,32.5)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "0.2"
%	 right-arrow= "head"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(110,105)
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(22,81)(96,14)
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,53)(102,53)(102,57)(98,57)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,45){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,33)(102,33)(102,37)(98,37)
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,73)(102,73)(102,77)(98,77)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,65){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,85.62)(95.62,76.88)
\psline[linewidth=0.2,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,64.38)(96.25,56.25)
\psline[linewidth=0.2,border=1.1,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,62.5)(96.25,36.88)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,85){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,25){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23,82)(95,40)
\psline[linewidth=0.2,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(22.5,6.88)(96.88,51.88)
\psline[linewidth=0.2,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,46.88)(96.25,73.12)
\psline[linewidth=0.2,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.38,45.12)(96.25,55)
\psline[linewidth=0.2,border=0.85,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.75,65.62)(96.62,74.38)
\psline[linewidth=0.2,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,23.75)(96.25,33.75)
\psline[linewidth=0.2,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,26.88)(96.88,71.25)
\psline[linewidth=0.2,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.38,25.12)(96.25,53.75)
\rput(10,85){$\ha$}
\rput(10,65){$\hb$}
\rput(10,45){$\hc$}
\rput(10,25){$\hd$}
\rput(110,75){$\hI$}
\rput(110,55){$\hII$}
\rput(110,35){$\hIII$}
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,13)(102,13)(102,17)(98,17)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,5){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\psline[linewidth=0.2,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,3.75)(96.88,13.75)
\rput(10,5){$\he$}
\rput(110,15){$\hIV$}
\rput(100,105){\trustees}
\rput(20,105){\trustors}
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23,84)(96.25,57.5)
\psline[linewidth=0.2,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,43.75)(96.26,35.63)
\psline[linewidth=0.2,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,5.62)(96.88,32.5)
\end{pspicture}


==> PIC/trust-net-2.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Apr 08 23:25:33 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="10" x-max="110" y-min="3" y-max="105" auto-bounding="true">
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(22,81);(22,81);(96.88,16.25);(96.88,16.25)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<parallelogram p3= "(102,57)"
%	 fill-style= "solid"
%	 p2= "(102,53)"
%	 fill-color= "#0000ff"
%	 p1= "(98,53)"
%	 stroke-color= "#0000ff"
%	 />
%<ellipse p3= "(21.5,47)"
%	 fill-style= "solid"
%	 p2= "(21.5,43)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,43)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<parallelogram p3= "(102,37)"
%	 fill-style= "solid"
%	 p2= "(102,33)"
%	 fill-color= "#0000ff"
%	 p1= "(98,33)"
%	 stroke-color= "#0000ff"
%	 />
%<parallelogram p3= "(102,77)"
%	 fill-style= "solid"
%	 p2= "(102,73)"
%	 fill-color= "#0000ff"
%	 p1= "(98,73)"
%	 stroke-color= "#0000ff"
%	 />
%<ellipse p3= "(21.5,67)"
%	 fill-style= "solid"
%	 p2= "(21.5,63)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,63)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,85.62);(23.12,85.62);(95.62,76.88);(95.62,76.88)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 points= "(23.12,64.38);(23.12,64.38);(96.25,56.25);(96.25,56.25)"
%	 arrow-head-width-minimum= "1.45"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "1.1"
%	 points= "(23.12,62.5);(23.12,62.5);(96.25,36.88);(96.25,36.88)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<ellipse p3= "(21.5,87)"
%	 fill-style= "solid"
%	 p2= "(21.5,83)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,83)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(21.5,27)"
%	 fill-style= "solid"
%	 p2= "(21.5,23)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,23)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23,82);(23,82);(95,40);(95,40)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(22.5,6.88);(22.5,6.88);(96.88,51.88);(96.88,51.88)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,46.88);(23.12,46.88);(96.25,73.12);(96.25,73.12)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.38,45.12);(23.38,45.12);(96.25,55);(96.25,55)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.85"
%	 points= "(23.75,65.62);(23.75,65.62);(96.62,74.38);(96.62,74.38)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,23.75);(23.12,23.75);(96.25,33.75);(96.25,33.75)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,26.88);(23.12,26.88);(96.88,71.25);(96.88,71.25)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.38,25.12);(23.38,25.12);(96.25,53.75);(96.25,53.75)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ha$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hb$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hc$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hI$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hII$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hIII$
%</text>
%<parallelogram p3= "(102,17)"
%	 fill-style= "solid"
%	 p2= "(102,13)"
%	 fill-color= "#0000ff"
%	 p1= "(98,13)"
%	 stroke-color= "#0000ff"
%	 />
%<ellipse p3= "(21.5,7)"
%	 fill-style= "solid"
%	 p2= "(21.5,3)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,3)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,3.75);(23.12,3.75);(96.25,14.38);(96.25,14.38)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\he$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hIV$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\trustees
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\trustors
%</text>
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23,84);(23,84);(96.25,57.5);(96.25,57.5)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,43.75);(23.12,43.75);(96.26,35.63);(96.26,35.63)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,5.62);(23.12,5.62);(96.88,32.5);(96.88,32.5)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(110,105)
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(22,81)(96.88,16.25)
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,53)(102,53)(102,57)(98,57)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,45){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,33)(102,33)(102,37)(98,37)
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,73)(102,73)(102,77)(98,77)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,65){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,85.62)(95.62,76.88)
\psline[arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,64.38)(96.25,56.25)
\psline[border=1.1,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,62.5)(96.25,36.88)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,85){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,25){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23,82)(95,40)
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(22.5,6.88)(96.88,51.88)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,46.88)(96.25,73.12)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.38,45.12)(96.25,55)
\psline[border=0.85,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.75,65.62)(96.62,74.38)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,23.75)(96.25,33.75)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,26.88)(96.88,71.25)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.38,25.12)(96.25,53.75)
\rput(10,85){$\ha$}
\rput(10,65){$\hb$}
\rput(10,45){$\hc$}
\rput(10,25){$\hd$}
\rput(110,75){$\hI$}
\rput(110,55){$\hII$}
\rput(110,35){$\hIII$}
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,13)(102,13)(102,17)(98,17)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,5){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,3.75)(96.25,14.38)
\rput(10,5){$\he$}
\rput(110,15){$\hIV$}
\rput(100,105){\trustees}
\rput(20,105){\trustors}
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23,84)(96.25,57.5)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,43.75)(96.26,35.63)
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,5.62)(96.88,32.5)
\end{pspicture}


==> PIC/trust-net-3.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Apr 08 23:26:54 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="10" x-max="110" y-min="3" y-max="105" auto-bounding="true">
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(22,81);(22,81);(96,14);(96,14)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<parallelogram p3= "(102,57)"
%	 fill-style= "solid"
%	 p2= "(102,53)"
%	 fill-color= "#0000ff"
%	 p1= "(98,53)"
%	 stroke-color= "#0000ff"
%	 />
%<ellipse p3= "(21.5,47)"
%	 fill-style= "solid"
%	 p2= "(21.5,43)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,43)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<parallelogram p3= "(102,37)"
%	 fill-style= "solid"
%	 p2= "(102,33)"
%	 fill-color= "#0000ff"
%	 p1= "(98,33)"
%	 stroke-color= "#0000ff"
%	 />
%<parallelogram p3= "(102,77)"
%	 fill-style= "solid"
%	 p2= "(102,73)"
%	 fill-color= "#0000ff"
%	 p1= "(98,73)"
%	 stroke-color= "#0000ff"
%	 />
%<ellipse p3= "(21.5,67)"
%	 fill-style= "solid"
%	 p2= "(21.5,63)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,63)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,85.62);(23.12,85.62);(95.62,76.88);(95.62,76.88)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 points= "(23.12,64.38);(23.12,64.38);(96.25,56.25);(96.25,56.25)"
%	 arrow-head-width-minimum= "1.45"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "1.1"
%	 points= "(23.12,62.5);(23.12,62.5);(96.25,36.88);(96.25,36.88)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<ellipse p3= "(21.5,87)"
%	 fill-style= "solid"
%	 p2= "(21.5,83)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,83)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(21.5,27)"
%	 fill-style= "solid"
%	 p2= "(21.5,23)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,23)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23,82);(23,82);(95,40);(95,40)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(22.5,6.88);(22.5,6.88);(96.88,51.88);(96.88,51.88)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,46.88);(23.12,46.88);(96.25,73.12);(96.25,73.12)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.38,45.12);(23.38,45.12);(96.25,55);(96.25,55)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.85"
%	 points= "(23.75,65.62);(23.75,65.62);(96.62,74.38);(96.62,74.38)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,23.75);(23.12,23.75);(96.25,33.75);(96.25,33.75)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,26.88);(23.12,26.88);(96.88,71.25);(96.88,71.25)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.38,25.12);(23.38,25.12);(96.25,53.75);(96.25,53.75)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ha$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hb$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hc$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hI$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hII$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hIII$
%</text>
%<parallelogram p3= "(102,17)"
%	 fill-style= "solid"
%	 p2= "(102,13)"
%	 fill-color= "#0000ff"
%	 p1= "(98,13)"
%	 stroke-color= "#0000ff"
%	 />
%<ellipse p3= "(21.5,7)"
%	 fill-style= "solid"
%	 p2= "(21.5,3)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,3)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,3.75);(23.12,3.75);(96.88,13.75);(96.88,13.75)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\he$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hIV$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\trustees
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\trustors
%</text>
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23,84);(23,84);(96.25,57.5);(96.25,57.5)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,43.75);(23.12,43.75);(96.26,35.63);(96.26,35.63)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,5.62);(23.12,5.62);(96.88,32.5);(96.88,32.5)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(110,105)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(22,81)(96,14)
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,53)(102,53)(102,57)(98,57)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,45){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,33)(102,33)(102,37)(98,37)
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,73)(102,73)(102,77)(98,77)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,65){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,85.62)(95.62,76.88)
\psline[linewidth=1.5,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,64.38)(96.25,56.25)
\psline[linewidth=1.5,border=1.1,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,62.5)(96.25,36.88)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,85){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,25){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23,82)(95,40)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(22.5,6.88)(96.88,51.88)
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,46.88)(96.25,73.12)
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.38,45.12)(96.25,55)
\psline[linewidth=1.5,border=0.85,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.75,65.62)(96.62,74.38)
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,23.75)(96.25,33.75)
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,26.88)(96.88,71.25)
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.38,25.12)(96.25,53.75)
\rput(10,85){$\ha$}
\rput(10,65){$\hb$}
\rput(10,45){$\hc$}
\rput(10,25){$\hd$}
\rput(110,75){$\hI$}
\rput(110,55){$\hII$}
\rput(110,35){$\hIII$}
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,13)(102,13)(102,17)(98,17)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,5){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,3.75)(96.88,13.75)
\rput(10,5){$\he$}
\rput(110,15){$\hIV$}
\rput(100,105){\trustees}
\rput(20,105){\trustors}
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23,84)(96.25,57.5)
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,43.75)(96.26,35.63)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,5.62)(96.88,32.5)
\end{pspicture}


==> PIC/trust-net-4.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Wed Apr 08 23:27:59 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="10" x-max="110" y-min="3" y-max="105" auto-bounding="true">
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(22,81);(22,81);(96,14);(96,14)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<parallelogram p3= "(102,57)"
%	 fill-style= "solid"
%	 p2= "(102,53)"
%	 fill-color= "#0000ff"
%	 p1= "(98,53)"
%	 stroke-color= "#0000ff"
%	 />
%<ellipse p3= "(21.5,47)"
%	 fill-style= "solid"
%	 p2= "(21.5,43)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,43)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<parallelogram p3= "(102,37)"
%	 fill-style= "solid"
%	 p2= "(102,33)"
%	 fill-color= "#0000ff"
%	 p1= "(98,33)"
%	 stroke-color= "#0000ff"
%	 />
%<parallelogram p3= "(102,77)"
%	 fill-style= "solid"
%	 p2= "(102,73)"
%	 fill-color= "#0000ff"
%	 p1= "(98,73)"
%	 stroke-color= "#0000ff"
%	 />
%<ellipse p3= "(21.5,67)"
%	 fill-style= "solid"
%	 p2= "(21.5,63)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,63)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,85.62);(23.12,85.62);(95.62,76.88);(95.62,76.88)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 points= "(23.12,64.38);(23.12,64.38);(96.25,56.25);(96.25,56.25)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "1.1"
%	 points= "(23.12,62.5);(23.12,62.5);(96.25,36.88);(96.25,36.88)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<ellipse p3= "(21.5,87)"
%	 fill-style= "solid"
%	 p2= "(21.5,83)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,83)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(21.5,27)"
%	 fill-style= "solid"
%	 p2= "(21.5,23)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,23)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23,82);(23,82);(95,40);(95,40)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(22.5,6.88);(22.5,6.88);(96.88,51.88);(96.88,51.88)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,46.88);(23.12,46.88);(96.25,73.12);(96.25,73.12)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.38,45.12);(23.38,45.12);(96.25,55);(96.25,55)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.85"
%	 points= "(23.75,65.62);(23.75,65.62);(96.62,74.38);(96.62,74.38)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,23.75);(23.12,23.75);(96.25,33.75);(96.25,33.75)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,26.88);(23.12,26.88);(96.88,71.25);(96.88,71.25)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.38,25.12);(23.38,25.12);(96.25,53.75);(96.25,53.75)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ha$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hb$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hc$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hI$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hII$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hIII$
%</text>
%<parallelogram p3= "(102,17)"
%	 fill-style= "solid"
%	 p2= "(102,13)"
%	 fill-color= "#0000ff"
%	 p1= "(98,13)"
%	 stroke-color= "#0000ff"
%	 />
%<ellipse p3= "(21.5,7)"
%	 fill-style= "solid"
%	 p2= "(21.5,3)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,3)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,3.75);(23.12,3.75);(96.88,13.75);(96.88,13.75)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\he$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hIV$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\trustees
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\trustors
%</text>
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23,84);(23,84);(96.25,57.5);(96.25,57.5)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,43.75);(23.12,43.75);(96.26,35.63);(96.26,35.63)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,5.62);(23.12,5.62);(96.88,32.5);(96.88,32.5)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 stroke-width= "1.5"
%	 right-arrow= "head"
%	 />
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(110,105)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(22,81)(96,14)
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,53)(102,53)(102,57)(98,57)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,45){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,33)(102,33)(102,37)(98,37)
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,73)(102,73)(102,77)(98,77)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,65){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,85.62)(95.62,76.88)
\psline[linewidth=1.5,border=0.3,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,64.38)(96.25,56.25)
\psline[linewidth=1.5,border=1.1,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,62.5)(96.25,36.88)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,85){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,25){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23,82)(95,40)
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(22.5,6.88)(96.88,51.88)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,46.88)(96.25,73.12)
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.38,45.12)(96.25,55)
\psline[border=0.85,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.75,65.62)(96.62,74.38)
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,23.75)(96.25,33.75)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,26.88)(96.88,71.25)
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.38,25.12)(96.25,53.75)
\rput(10,85){$\ha$}
\rput(10,65){$\hb$}
\rput(10,45){$\hc$}
\rput(10,25){$\hd$}
\rput(110,75){$\hI$}
\rput(110,55){$\hII$}
\rput(110,35){$\hIII$}
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,13)(102,13)(102,17)(98,17)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,5){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,3.75)(96.88,13.75)
\rput(10,5){$\he$}
\rput(110,15){$\hIV$}
\rput(100,105){\trustees}
\rput(20,105){\trustors}
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23,84)(96.25,57.5)
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,43.75)(96.26,35.63)
\psline[linewidth=1.5,border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,5.62)(96.88,32.5)
\end{pspicture}


==> PIC/trust-net.tex <==
%%Created by jPicEdt 1.4.1_03: mixed JPIC-XML/LaTeX format
%%Tue Feb 18 16:50:37 GMT-10:00 2020
%%Begin JPIC-XML
%<?xml version="1.0" standalone="yes"?>
%<jpic x-min="10" x-max="110" y-min="3" y-max="105" auto-bounding="true">
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(22,81);(22,81);(96,14);(96,14)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<parallelogram p3= "(102,57)"
%	 fill-style= "solid"
%	 p2= "(102,53)"
%	 fill-color= "#0000ff"
%	 p1= "(98,53)"
%	 stroke-color= "#0000ff"
%	 />
%<ellipse p3= "(21.5,47)"
%	 fill-style= "solid"
%	 p2= "(21.5,43)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,43)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<parallelogram p3= "(102,37)"
%	 fill-style= "solid"
%	 p2= "(102,33)"
%	 fill-color= "#0000ff"
%	 p1= "(98,33)"
%	 stroke-color= "#0000ff"
%	 />
%<parallelogram p3= "(102,77)"
%	 fill-style= "solid"
%	 p2= "(102,73)"
%	 fill-color= "#0000ff"
%	 p1= "(98,73)"
%	 stroke-color= "#0000ff"
%	 />
%<ellipse p3= "(21.5,67)"
%	 fill-style= "solid"
%	 p2= "(21.5,63)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,63)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,85.62);(23.12,85.62);(95.62,76.88);(95.62,76.88)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 points= "(23.12,64.38);(23.12,64.38);(96.25,56.25);(96.25,56.25)"
%	 arrow-head-width-minimum= "1.45"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "1.1"
%	 points= "(23.12,62.5);(23.12,62.5);(96.25,36.88);(96.25,36.88)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(30,59)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\five$
%</text>
%<ellipse p3= "(21.5,87)"
%	 fill-style= "solid"
%	 p2= "(21.5,83)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,83)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<ellipse p3= "(21.5,27)"
%	 fill-style= "solid"
%	 p2= "(21.5,23)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,23)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23,82);(23,82);(95,40);(95,40)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(22.5,6.88);(22.5,6.88);(96.88,51.88);(96.88,51.88)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,46.88);(23.12,46.88);(96.25,73.12);(96.25,73.12)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.38,45.12);(23.38,45.12);(96.25,55);(96.25,55)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.85"
%	 points= "(23.75,65.62);(23.75,65.62);(96.62,74.38);(96.62,74.38)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,23.75);(23.12,23.75);(96.25,33.75);(96.25,33.75)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,26.88);(23.12,26.88);(96.88,71.25);(96.88,71.25)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.38,25.12);(23.38,25.12);(96.25,53.75);(96.25,53.75)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(30,50.62)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\six$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(42.5,48.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\seven$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(30,41.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eight$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(29.38,31.25)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\nine$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(31.88,23.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\eleven$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(48.12,34.38)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\ten$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,85)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\ha$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,65)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hb$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,45)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hc$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,25)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hd$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hI$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,55)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hII$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,35)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hIII$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(30,86)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\one$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(29.38,67.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\three$
%</text>
%<parallelogram p3= "(102,17)"
%	 fill-style= "solid"
%	 p2= "(102,13)"
%	 fill-color= "#0000ff"
%	 p1= "(98,13)"
%	 stroke-color= "#0000ff"
%	 />
%<ellipse p3= "(21.5,7)"
%	 fill-style= "solid"
%	 p2= "(21.5,3)"
%	 fill-color= "#ff6666"
%	 p1= "(18.5,3)"
%	 closure= "open"
%	 angle-end= "0"
%	 stroke-color= "#ff6666"
%	 angle-start= "0"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,3.75);(23.12,3.75);(96.88,13.75);(96.88,13.75)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(10,5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\he$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(110,15)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\hIV$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(100,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\trustees
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(20,105)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%\trustors
%</text>
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23,84);(23,84);(96.25,57.5);(96.25,57.5)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,43.75);(23.12,43.75);(96.26,35.63);(96.26,35.63)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<multicurve fill-style= "none"
%	 arrow-global-scale-length= "1.45"
%	 stroke-overstrike-width= "0.75"
%	 points= "(23.12,5.62);(23.12,5.62);(96.88,32.5);(96.88,32.5)"
%	 arrow-head-width-minimum= "1.45"
%	 stroke-overstrike= "true"
%	 arrow-head-length-scale= "1.55"
%	 right-arrow= "head"
%	 />
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(30,11.88)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\twelve$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(30.62,3.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\fourteen$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(44.38,12.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\thirteen$
%</text>
%<text text-vert-align= "top"
%	 fill-style= "none"
%	 anchor-point= "(25,78)"
%	 text-frame= "noframe"
%	 text-hor-align= "right"
%	 >
%$\fifteen$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(50,75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\two$
%</text>
%<text text-vert-align= "baseline"
%	 fill-style= "none"
%	 anchor-point= "(38.12,73.75)"
%	 text-frame= "noframe"
%	 text-hor-align= "left"
%	 >
%$\sixteen$
%</text>
%<text text-vert-align= "bottom"
%	 fill-style= "none"
%	 anchor-point= "(46.88,62.5)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\four$
%</text>
%<text text-vert-align= "center-v"
%	 fill-style= "none"
%	 anchor-point= "(70,90)"
%	 text-frame= "noframe"
%	 text-hor-align= "center-h"
%	 >
%$\namr$
%</text>
%</jpic>
%%End JPIC-XML
%PSTricks content-type (pstricks.sty package needed)
%Add \usepackage{pstricks} in the preamble of your LaTeX file
%You can rescale the whole picture (to 80% for instance) by using the command \def\JPicScale{0.8}
\ifx\JPicScale\undefined\def\JPicScale{1}\fi
\psset{unit=\JPicScale mm}
\psset{linewidth=0.3,dotsep=1,hatchwidth=0.3,hatchsep=1.5,shadowsize=1,dimen=middle}
\psset{dotsize=0.7 2.5,dotscale=1 1,fillcolor=black}
\psset{arrowsize=1 2,arrowlength=1,arrowinset=0.25,tbarsize=0.7 5,bracketlength=0.15,rbracketlength=0.15}
\begin{pspicture}(0,0)(110,105)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(22,81)(96,14)
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,53)(102,53)(102,57)(98,57)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,45){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,33)(102,33)(102,37)(98,37)
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,73)(102,73)(102,77)(98,77)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,65){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,85.62)(95.62,76.88)
\psline[arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,64.38)(96.25,56.25)
\psline[border=1.1,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,62.5)(96.25,36.88)
\rput[t](30,59){$\five$}
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,85){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,25){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23,82)(95,40)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(22.5,6.88)(96.88,51.88)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,46.88)(96.25,73.12)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.38,45.12)(96.25,55)
\psline[border=0.85,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.75,65.62)(96.62,74.38)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,23.75)(96.25,33.75)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,26.88)(96.88,71.25)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.38,25.12)(96.25,53.75)
\rput[b](30,50.62){$\six$}
\rput[b](42.5,48.75){$\seven$}
\rput[t](30,41.25){$\eight$}
\rput[br](29.38,31.25){$\nine$}
\rput[t](31.88,23.75){$\eleven$}
\rput[tl](48.12,34.38){$\ten$}
\rput(10,85){$\ha$}
\rput(10,65){$\hb$}
\rput(10,45){$\hc$}
\rput(10,25){$\hd$}
\rput(110,75){$\hI$}
\rput(110,55){$\hII$}
\rput(110,35){$\hIII$}
\rput[b](30,86){$\one$}
\rput[b](29.38,67.5){$\three$}
\pspolygon[linecolor=blue,fillcolor=blue,fillstyle=solid](98,13)(102,13)(102,17)(98,17)
\newrgbcolor{userLineColour}{1 0.4 0.4}
\newrgbcolor{userFillColour}{1 0.4 0.4}
\rput{90}(20,5){\psellipse[linecolor=userLineColour,fillcolor=userFillColour,fillstyle=solid](0,0)(2,1.5)}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,3.75)(96.88,13.75)
\rput(10,5){$\he$}
\rput(110,15){$\hIV$}
\rput(100,105){\trustees}
\rput(20,105){\trustors}
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23,84)(96.25,57.5)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,43.75)(96.26,35.63)
\psline[border=0.75,arrowscale=1 1.45,arrowsize=1.45 2,arrowlength=1.55]{->}(23.12,5.62)(96.88,32.5)
\rput[br](30,11.88){$\twelve$}
\rput[t](30.62,3.75){$\fourteen$}
\rput[tl](44.38,12.5){$\thirteen$}
\rput[tr](25,78){$\fifteen$}
\rput[bl](50,75){$\two$}
\rput[Bl](38.12,73.75){$\sixteen$}
\rput[b](46.88,62.5){$\four$}
\rput(70,90){$\namr$}
\end{pspicture}


==> macros-nuc-lmcs.tex <==
% !TEX root = 00-nuc-lmcs.tex
%!TEX TS-program = xelatex
%!TEX encoding = UTF-8 Unicode


%\usepackage{etex}
%\usepackage{hyperref} 
\usepackage{tikz-cd}
\tikzcdset{
  shift left/.default=+0.7ex,% default: +0.56ex
  shift right/.default=+0.7ex}
  
  \tikzcdset{arrow style=tikz,
  diagrams={>={Straight Barb[scale=0.8]}}}


\newenvironment{tikzar}[1][]{{}\kern-4pt\begin{tikzcd}[ampersand replacement=\&,#1]}%
{\end{tikzcd}\kern-4pt{}}

\usetikzlibrary{cd}
\usetikzlibrary{decorations.pathmorphing,positioning}

\usepackage{pstricks}
\usepackage{amssymb}
\usepackage{amsmath}
%\usepackage{amsthm}
\usepackage{txfonts}
\usepackage{bbm}
\usepackage[only,bigcurlywedge,bigcurlyvee]{stmaryrd}
\usepackage{enumitem}
\usepackage{fullpage}
\usepackage{multicol}

\RequirePackage[T1]{fontenc}
\usepackage[utf8]{inputenc}



\def\pushright#1{{%              set up
    \parfillskip=0pt            % so \par doesnt push \square to left
    \widowpenalty=10000         % so we dont break the page before \square
    \displaywidowpenalty=10000  % ditto
    \finalhyphendemerits=0      % TeXbook exercise 14.32
   %
   %                 horizontal
    \leavevmode                 % \nobreak means lines not pages
    \unskip                     % remove previous space or glue
    \nobreak                    % don't break lines
    \hfil                       % ragged right if we spill over
    \penalty50                  % discouragement to do so
    \hskip.2em                  % ensure some space
    \null                       % anchor following \hfill
    \hfill                      % push \square to right
    {#1}                        % the end-of-proof mark (or whatever)
   %
   %                   vertical
    \par}}                      % build paragraph

 % prefer proofs with statements, also space after
\def\qed{\pushright{$\square$}\penalty-700 \smallskip}
\newenvironment{prf}[1]{\begin{trivlist} \item[{\bf ~Proof}#1.]}%
{\qed\end{trivlist}}

\newcommand{\bpr}{\begin{prf}{}}
\newcommand{\epr}{\end{prf}}
\newcommand{\bprf}[1]{\begin{prf}{#1}}
\newcommand{\eprf}{\end{prf}}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{example}[theorem]{Example}
\newtheorem{definition}[theorem]{Definition}
%\theoremstyle{remark}
%\newtheorem*{remark}{Remark}

\def\introrule{{\mathcal I}}
\def\elimrule{{\mathcal E}}%%
\def\andintro{\using{\land}
\introrule\justifies}%%
\def\impelim{\using{\Rightarrow}\elimrule\justifies}%%
\def\allintro{\using{\forall}\introrule\justifies}%%
\def\allelim{\using{\forall}\elimrule\justifies}%%
\def\falseelim{\using{\bot}\elimrule\justifies}%%
\def\existsintro{\using{\exists}\introrule\justifies}%%

%% #1 is meant to be 1 or 2 for the first or second formula
\def\andelim#1{\using{\land}#1\elimrule\justifies}%%
\def\orintro#1{\using{\lor}#1\introrule\justifies}%%

%% #1 is meant to be a label corresponding to the discharged hypothesis/es
\def\impintro#1{\using{\Rightarrow}\introrule_{#1}\justifies}%%
\def\orelim#1{\using{\lor}\elimrule_{#1}\justifies}%%
\def\existselim#1{\using{\exists}\elimrule_{#1}\justifies}

%%==========================================================================

\newdimen\proofrulebreadth \proofrulebreadth=.05em
\newdimen\proofdotseparation \proofdotseparation=1.25ex
\newdimen\proofrulebaseline \proofrulebaseline=2ex
\newcount\proofdotnumber \proofdotnumber=3
\let\then\relax
\def\hfi{\hskip0pt plus.0001fil}
\mathchardef\squigto="3A3B
%
% flag where we are
\newif\ifinsideprooftree\insideprooftreefalse
\newif\ifonleftofproofrule\onleftofproofrulefalse
\newif\ifproofdots\proofdotsfalse
\newif\ifdoubleproof\doubleprooffalse
\let\wereinproofbit\relax
%
% dimensions and boxes of bits
\newdimen\shortenproofleft
\newdimen\shortenproofright
\newdimen\proofbelowshift
\newbox\proofabove
\newbox\proofbelow
\newbox\proofrulename
%
% miscellaneous commands for setting values
\def\shiftproofbelow{\let\next\relax\afterassignment\setshiftproofbelow\dimen0 }
\def\shiftproofbelowneg{\def\next{\multiply\dimen0 by-1 }%
\afterassignment\setshiftproofbelow\dimen0 }
\def\setshiftproofbelow{\next\proofbelowshift=\dimen0 }
\def\setproofrulebreadth{\proofrulebreadth}

%=============================================================================
\def\prooftree{% NESTED ZERO (\ifonleftofproofrule)
%
% first find out whether we're at the left-hand end of a proof rule
\ifnum  \lastpenalty=1
\then   \unpenalty
\else   \onleftofproofrulefalse
\fi
%
% some space on left (except if we're on left, and no infinity for outermost)
\ifonleftofproofrule
\else   \ifinsideprooftree
        \then   \hskip.5em plus1fil
        \fi
\fi
%
% begin our proof tree environment
\bgroup% NESTED ONE (\proofbelow, \proofrulename, \proofabove,
%               \shortenproofleft, \shortenproofright, \proofrulebreadth)
\setbox\proofbelow=\hbox{}\setbox\proofrulename=\hbox{}%
\let\justifies\proofover\let\leadsto\proofoverdots\let\Justifies\proofoverdbl
\let\using\proofusing\let\[\prooftree
\ifinsideprooftree\let\]\endprooftree\fi
\proofdotsfalse\doubleprooffalse
\let\thickness\setproofrulebreadth
\let\shiftright\shiftproofbelow \let\shift\shiftproofbelow
\let\shiftleft\shiftproofbelowneg
\let\ifwasinsideprooftree\ifinsideprooftree
\insideprooftreetrue
%
% now begin to set the top of the rule (definitions local to it)
\setbox\proofabove=\hbox\bgroup$\displaystyle % NESTED TWO
\let\wereinproofbit\prooftree
%
% these local variables will be copied out:
\shortenproofleft=0pt \shortenproofright=0pt \proofbelowshift=0pt
%
% flags to enable inner proof tree to detect if on left:
\onleftofproofruletrue\penalty1
}

%=============================================================================
% end whatever box and copy crucial values out of it
\def\eproofbit{% NESTED TWO
%
% various hacks applicable to hypothesis list 
\ifx    \wereinproofbit\prooftree
\then   \ifcase \lastpenalty
        \then   \shortenproofright=0pt  % 0: some other object, no indentation
        \or     \unpenalty\hfil         % 1: empty hypotheses, just glue
        \or     \unpenalty\unskip       % 2: just had a tree, remove glue
        \else   \shortenproofright=0pt  % eh?
        \fi
\fi
%
% pass out crucial values from scope
\global\dimen0=\shortenproofleft
\global\dimen1=\shortenproofright
\global\dimen2=\proofrulebreadth
\global\dimen3=\proofbelowshift
\global\dimen4=\proofdotseparation
\global\count255=\proofdotnumber
%
% end the box
$\egroup  % NESTED ONE
%
% restore the values
\shortenproofleft=\dimen0
\shortenproofright=\dimen1
\proofrulebreadth=\dimen2
\proofbelowshift=\dimen3
\proofdotseparation=\dimen4
\proofdotnumber=\count255
}

%=============================================================================
\def\proofover{% NESTED TWO
\eproofbit % NESTED ONE
\setbox\proofbelow=\hbox\bgroup % NESTED TWO
\let\wereinproofbit\proofover
$\displaystyle
}%
%
%=============================================================================
\def\proofoverdbl{% NESTED TWO
\eproofbit % NESTED ONE
\doubleprooftrue
\setbox\proofbelow=\hbox\bgroup % NESTED TWO
\let\wereinproofbit\proofoverdbl
$\displaystyle
}%
%
%=============================================================================
\def\proofoverdots{% NESTED TWO
\eproofbit % NESTED ONE
\proofdotstrue
\setbox\proofbelow=\hbox\bgroup % NESTED TWO
\let\wereinproofbit\proofoverdots
$\displaystyle
}%
%
%=============================================================================
\def\proofusing{% NESTED TWO
\eproofbit % NESTED ONE
\setbox\proofrulename=\hbox\bgroup % NESTED TWO
\let\wereinproofbit\proofusing
\kern0.3em$
}

%=============================================================================
\def\endprooftree{% NESTED TWO
\eproofbit % NESTED ONE
% \dimen0 =     length of proof rule
% \dimen1 =     indentation of conclusion wrt rule
% \dimen2 =     new \shortenproofleft, ie indentation of conclusion
% \dimen3 =     new \shortenproofright, ie
%                space on right of conclusion to end of tree
% \dimen4 =     space on right of conclusion below rule
  \dimen5 =0pt% spread of hypotheses
% \dimen6, \dimen7 = height & depth of rule
%
% length of rule needed by proof above
\dimen0=\wd\proofabove \advance\dimen0-\shortenproofleft
\advance\dimen0-\shortenproofright
%
% amount of spare space below
\dimen1=.5\dimen0 \advance\dimen1-.5\wd\proofbelow
\dimen4=\dimen1
\advance\dimen1\proofbelowshift \advance\dimen4-\proofbelowshift
%
% conclusion sticks out to left of immediate hypotheses
\ifdim  \dimen1<0pt
\then   \advance\shortenproofleft\dimen1
        \advance\dimen0-\dimen1
        \dimen1=0pt
%       now it sticks out to left of tree!
        \ifdim  \shortenproofleft<0pt
        \then   \setbox\proofabove=\hbox{%
                        \kern-\shortenproofleft\unhbox\proofabove}%
                \shortenproofleft=0pt
        \fi
\fi
%
% and to the right
\ifdim  \dimen4<0pt
\then   \advance\shortenproofright\dimen4
        \advance\dimen0-\dimen4
        \dimen4=0pt
\fi
%
% make sure enough space for label
\ifdim  \shortenproofright<\wd\proofrulename
\then   \shortenproofright=\wd\proofrulename
\fi
%
% calculate new indentations
\dimen2=\shortenproofleft \advance\dimen2 by\dimen1
\dimen3=\shortenproofright\advance\dimen3 by\dimen4
%
% make the rule or dots, with name attached
\ifproofdots
\then
        \dimen6=\shortenproofleft \advance\dimen6 .5\dimen0
        \setbox1=\vbox to\proofdotseparation{\vss\hbox{$\cdot$}\vss}%
        \setbox0=\hbox{%
                \advance\dimen6-.5\wd1
                \kern\dimen6
                $\vcenter to\proofdotnumber\proofdotseparation
                        {\leaders\box1\vfill}$%
                \unhbox\proofrulename}%
\else   \dimen6=\fontdimen22\the\textfont2 % height of maths axis
        \dimen7=\dimen6
        \advance\dimen6by.5\proofrulebreadth
        \advance\dimen7by-.5\proofrulebreadth
        \setbox0=\hbox{%
                \kern\shortenproofleft
                \ifdoubleproof
                \then   \hbox to\dimen0{%
                        $\mathsurround0pt\mathord=\mkern-6mu%
                        \cleaders\hbox{$\mkern-2mu=\mkern-2mu$}\hfill
                        \mkern-6mu\mathord=$}%
                \else   \vrule height\dimen6 depth-\dimen7 width\dimen0
                \fi
                \unhbox\proofrulename}%
        \ht0=\dimen6 \dp0=-\dimen7
\fi
%
% set up to centre outermost tree only
\let\doll\relax
\ifwasinsideprooftree
\then   \let\VBOX\vbox
\else   \ifmmode\else$\let\doll=$\fi
        \let\VBOX\vcenter
\fi
% this \vbox or \vcenter is the actual output:
\VBOX   {\baselineskip\proofrulebaseline \lineskip.2ex
        \expandafter\lineskiplimit\ifproofdots0ex\else-0.6ex\fi
        \hbox   spread\dimen5   {\hfi\unhbox\proofabove\hfi}%
        \hbox{\box0}%
        \hbox   {\kern\dimen2 \box\proofbelow}}\doll%
%
% pass new indentations out of scope
\global\dimen2=\dimen2
\global\dimen3=\dimen3
\egroup % NESTED ZERO
\ifonleftofproofrule
\then   \shortenproofleft=\dimen2
\fi
\shortenproofright=\dimen3
%
% some space on right and flag we've just made a tree
\onleftofproofrulefalse
\ifinsideprooftree
\then   \hskip.5em plus 1fil \penalty2
\fi
}
%% END PROOFTREE

% for Dominic comments
\definecolor{dominicred}{rgb}{0.85, 0.0, 0.0}
\newcommand\dominic[2][\rule{3ex}{4pt}]{{\color{dominicred}#2\marginpar{\color{dominicred}\centering\raggedleft\tiny#1}}}

\newcommand{\chc}[1]{{\left\lceil {#1}\right\rceil }}
\newcommand{\chcc}{\lceil\! \rceil}
\newcommand{\sfrac}[2]{\mbox{$\frac{#1}{#2}$}}
\newcommand{\mdls}[2]{\left({#1}\models {#2}\right)}
\newcommand{\mdl}[3]{{#1}\overset {#2}\models {#3}}
\newcommand{\mdll}[3]{\left({#1}\overset {#2}\models {#3}\right)}


% \newcommand{\PSt}{P}
% \newcommand{\PPSt}{\models}
\newcommand{\op}{{o}}
% \newcommand{\St}{P}
% \newcommand{\SSSbjh}{\widehat S}
% \newcommand{\OOObjh}{\widehat O}
% \newcommand{\SSbjh}{\Sigma}
% \newcommand{\OObjh}{\Theta}
% \newcommand{\Sbjh}{\Sigma}
% \newcommand{\Objh}{\Theta}

% \newcommand{\PSbj}{\BBb}
% \newcommand{\PObj}{\AAa}
\newcommand{\CoalgPhi}{(\Up\BBb)^{\Rmon\Phi}}
\newcommand{\AlgPhi}{(\Do\AAa)^{\Lmon\Phi}}
\newcommand{\CoalgH}{(\Up\CCc)^{\Rmon H}}
\newcommand{\AlgH}{(\Do\CCc)^{\Lmon H}}

\newcommand{\dual}{{\sharp}}
\newcommand{\ddual}{{\sharp\sharp}}
\newcommand*{\KEnv}[1]{\overline{#1}} % Cauchy completion


% \newcommand{\PSbjh}{\widehat{\sf S}}
% \newcommand{\PObjh}{\widehat{\sf O}}
% \newcommand{\SSbj}{S}
% \newcommand{\OObj}{O}
% \newcommand{\NNat}{N}
% \newcommand{\RRat}{R}
% \newcommand{\Nat}{\NNn}
% %\newcommand{\OOObj}{{\widehat{\OOO}}}
% %\newcommand{\SSSbj}{{\widehat{\SSS}}}
% \newcommand{\Obj}{{\OOo}}
% \newcommand{\Sbj}{{\SSs}}
% \newcommand{\Ent}{{\sf E}}
% \newcommand{\Rat}{{\sf R}}
% \newcommand{\Bin}{{\sf B}}
% \newcommand{\bind}{b}
% \newcommand{\bindd}{\beta}
% \newcommand{\Del}{{\sf D}}
% \newcommand{\del}{d}
% \newcommand{\dell}{\delta}
% \newcommand{\Tr}{{\rm tr}}
% \newcommand{\Prob}{\Pr}
% \newcommand{\Sim}{{\rm s}}
% \newcommand{\pthc}{\#}

\renewcommand{\to}{\xrightarrow{}}%{\longrightarrow}
\newcommand{\ot}{\xleftarrow{}}%{\longleftarrow}
\newcommand{\tto}[1]{\xrightarrow{#1}}
\newcommand{\oot}[1]{\xleftarrow{#1}}
\newcommand{\ttto}[2]{\xrightarrow[{#2}]{#1}}
\newcommand{\ooot}[2]{\xleftarrow[{#2}]{#1}}
\newcommand{\mono}{\rightarrowtail}
\newcommand{\epi}{\twoheadrightarrow}
\newcommand{\inclusion}{\hookrightarrow}
\newcommand{\mmono}[1]{\stackrel{#1}\rightarrowtail}
\newcommand{\eepi}[1]{\stackrel{#1}\twoheadrightarrow}
\newcommand{\iinclusion}[1]{\stackrel{#1}\hookrightarrow}
\newcommand{\longmapsfrom}{\mathrel{\reflectbox{\ensuremath{\longmapsto}}}}
\newcommand{\mapsfrom}{\mathrel{\reflectbox{\ensuremath{\mapsto}}}}
\newcommand{\pfn}{\rightharpoonup}
\newcommand{\ppfn}[1]{\stackrel{#1}\rightharpoonup}

\newcommand{\inup}{\mathbin{\rotatebox[origin=c]{90}{$\in$}}}


\newcommand{\WP}{\mbox{\Large $\wp$}}
\newcommand{\Wp}[1]{\WP{#1}}%
\newcommand{\Wpp}[1]{\WP^o{#1}}%{\WP^o\left({#1}\right)}
\newcommand{\fin}[1]{\dot{#1}}
\newcommand{\Set}{\mathsf{Set}}
\newcommand{\sSet}{\mathsf{sSet}}
\newcommand{\Hilb}{\mathsf{Hilb}}
\newcommand{\FHilb}{\fin{\mathsf H}\mathsf{ilb}}
\newcommand{\FSet}{\fin{\mathsf S}\mathsf{et}}
\newcommand{\SET}{\mathsf{SET}}
\newcommand{\Suj}{\mathsf{Suj}}
\newcommand{\Inj}{\mathsf{Inj}}
\newcommand{\Iso}{\mathsf{Iso}}
\newcommand{\Cat}{\mathsf{Cat}}
\newcommand{\CAT}{\mathsf{CAT}}
\newcommand{\Pos}{\mathsf{Pos}}
\newcommand{\Lin}{\mathsf{Lin}}
\newcommand{\Esp}{\mathsf{Esp}}
\newcommand{\Desc}{\mathsf{Desc}}
\newcommand{\Ab}{\mathsf{Ab}}


\newcommand{\AdjL}[1]{{#1}^\ast_\ast}
\newcommand{\MndL}{\MmM}%{\LLL}%
\newcommand{\CmnL}{\EeE}%{\UUU}%
\newcommand{\NucL}{{\lft \NnN}}%{\NNN}%
\newcommand{\NNucL}{\Kar\NucL}
\newcommand{\LucL}{{\rgt \NnN}}
\newcommand{\EMnd}{{\lft\EM}}
\newcommand{\ECmn}{{\lft\EC}}
\newcommand{\KMnd}{{\rgt\KM}}
\newcommand{\KCmn}{{\rgt\KC}}
\newcommand{\EEMnd}{\Kar\EMnd}
\newcommand{\EECmn}{\Kar\ECmn}
\newcommand{\KKMnd}{\Kar\KMnd}
\newcommand{\KKCmn}{\Kar\KCmn}


\newcommand{\Cut}[1]{\NucL_{0}{#1}}%{\DdD}%{\NNN\left({#1}\right)}

\newcommand{\MA}{{\sf MA}}
\newcommand{\AM}{{\sf AM}}
\newcommand{\AC}{{\sf AC}}
\newcommand{\EM}{{\sf EM}}
\newcommand{\KC}{{\sf KC}}
\newcommand{\EC}{{\sf EC}}
\newcommand{\KM}{{\sf KM}}
\newcommand{\MN}{{\sf MN}}
\newcommand{\CN}{{\sf CN}}
\newcommand{\NM}{{\sf NM}}
\newcommand{\NC}{{\sf NC}}




\newcommand{\Matrp}{\Mat_0}
\newcommand{\Adjp}{\Adj_0}
\newcommand{\Mndp}{\Mnd_0}
\newcommand{\Cmnp}{\Cmn_0}
\newcommand{\Nucp}{\Nucl_0}
\newcommand{\MAp}{\MA_0}
\newcommand{\AMp}{\AM_0}
\newcommand{\ACp}{\AC_0}
\newcommand{\EMp}{\EM_0}
\newcommand{\ECp}{\EC_0}
\newcommand{\KCp}{\KC_0}
\newcommand{\MNp}{\MN_0}
\newcommand{\CNp}{\CN_0}
\newcommand{\Matone}{\Mat_1}
\newcommand{\KK}{R}
\newcommand{\Adjone}{\Adj_1}
\newcommand{\Mndone}{\Mnd_1}
\newcommand{\Cmnone}{\Cmn_1}
\newcommand{\Nucone}{\Nucl_1}
\newcommand{\MAone}{\MA_1}
\newcommand{\AMone}{\AM_1}
\newcommand{\ACone}{\AC_1}
\newcommand{\EMone}{\EM_1}
\newcommand{\KCone}{\KC_1}
\newcommand{\MNone}{\MN_1}
\newcommand{\CNone}{\CN_1}


\newcommand{\Mattwo}{\Mat_2}%{\FMod \KK}
\newcommand{\Adjtwo}{\Adj_2}
\newcommand{\Mndtwo}{\Mnd_2}
\newcommand{\Cmntwo}{\Cmn_2}
\newcommand{\Nuctwo}{\Nucl_2}
\newcommand{\MAtwo}{\MA_2}
\newcommand{\AMtwo}{\AM_2}
\newcommand{\ACtwo}{\AC_2}
\newcommand{\EMtwo}{\EM_2}
\newcommand{\KCtwo}{\KC_2}
\newcommand{\MNtwo}{\MN_2}
\newcommand{\CNtwo}{\CN_2}

\newcommand{\Matthree}{\Mat_3}%{\FMod \KK}
\newcommand{\Adjthree}{\Adj_3}
\newcommand{\Mndthree}{\Mnd_3}
\newcommand{\Cmnthree}{\Cmn_3}
\newcommand{\Nucthree}{\Nucl_3}
\newcommand{\MAthree}{\MA_3}
\newcommand{\AMthree}{\AM_3}
\newcommand{\ACthree}{\AC_3}
\newcommand{\EMthree}{\EM_3}
\newcommand{\KCthree}{\KC_3}
\newcommand{\MNthree}{\MN_3}
\newcommand{\CNthree}{\CN_3}


\newcommand{\Matfour}{\Mat_4}%{\FMod \KK}
\newcommand{\Adjfour}{\Adj_4}
\newcommand{\Mndfour}{\Mnd_4}
\newcommand{\Cmnfour}{\Cmn_4}
\newcommand{\Nucfour}{\Nucl_4}
\newcommand{\MAfour}{\MA_4}
\newcommand{\MAafour}{\overrightarrow{\MA}_4}
\newcommand{\AMfour}{\AM_4}
\newcommand{\ACfour}{\AC_4}
\newcommand{\EMfour}{\EM_4}
\newcommand{\KCfour}{\KC_4}
\newcommand{\MNfour}{\MN_4}
\newcommand{\CNfour}{\CN_4}
\newcommand{\NMfour}{\NM_4}
\newcommand{\NCfour}{\NC_4}

\newcommand{\Matfive}{\Mat_5}%{\FMod \KK}
\newcommand{\Adjfive}{\Adj_5}
\newcommand{\Mndfive}{\Mnd_5}
\newcommand{\Cmnfive}{\Cmn_5}
\newcommand{\Nucfive}{\Nucl_5}
\newcommand{\MAfive}{\MA_5}
\newcommand{\MAafive}{\overrightarrow{\MA}_5}
\newcommand{\AMfive}{\AM_5}
\newcommand{\ACfive}{\AC_5}
\newcommand{\EMfive}{\EM_5}
\newcommand{\KCfive}{\KC_5}
\newcommand{\MNfive}{\MN_5}
\newcommand{\CNfive}{\CN_5}
\newcommand{\NMfive}{\NM_5}
\newcommand{\NCfive}{\NC_5}





\newcommand{\vsp}[1]{\KK^{{#1}}}
\newcommand{\lcomp}{\ ;}
\newcommand{\dashvdash}{\dashv\vdash}


\newcommand{\Mat}{\mathsf{Mat}}
\newcommand{\Adj}{\mathsf{Adj}}
\newcommand{\Mnd}{\mathsf{Mnd}}
\newcommand{\Cmn}{\mathsf{Cmn}}
\newcommand{\Adja}{\Kar{\mathsf{Adj}}}
\newcommand{\Mnda}{\Kar{\mathsf{Mnd}}}
\newcommand{\Cmna}{\Kar{\mathsf{Cmn}}}
\newcommand{\Nucl}{\mathsf{Nuc}}
\newcommand{\Lucl}{\mathsf{Luc}}
\newcommand{\Chu}{\mathsf{Chu}}
\newcommand{\chu}{\mathsf{chu}}
\newcommand{\SA}{\mathsf{CAK}}
\newcommand{\CAC}{\mathsf{CCh}}
\newcommand{\Rel}{\mathsf{Rel}}
\newcommand{\im}{\mathrm{im}}
\newcommand{\id}{\mathrm{id}}
\newcommand{\Id}{\mathrm{Id}}
\newcommand{\Dom}{\mathrm{Dom}}
\newcommand{\Cod}{\mathrm{Cod}}

%\newcommand{\nil}{\top}
%\newcommand{\blank}{\sqcup}

\newcommand{\REE}{\EEE^{\bullet}}
\newcommand{\RMM}{\MMM^{\bullet}}

\newcommand{\support}{{\rm supp}}
\renewcommand{\fact}{\wr}
\newcommand{\Fact}{\mbox{\Large$\wr$}}

\newcommand{\du}[1]{\KK^{#1}}
%{\left[{#1}|\KK\right]}%{{#1}\multimap\KK}%

%\newcommand{\Du}{\bot\hspace{-3mm}\raisebox{.5mm}{$\bot$}}

%\newcommand{\CKmatr}[2]{{#1}_{[{#2}]}}





\newcommand{\AAA}{{\mathcal A}}
\newcommand{\BBB}{{\mathcal B}}
\newcommand{\CCC}{{\mathcal C}}
\newcommand{\DDD}{{\mathcal D}}
\newcommand{\EEE}{{\mathcal E}}
\newcommand{\FFF}{{\mathcal F}}
\newcommand{\GGG}{{\mathcal G}}
\newcommand{\HHH}{{\mathcal H}}
\newcommand{\III}{{\mathcal I}}
\newcommand{\JJJ}{{\mathcal J}}
\newcommand{\KKK}{{\mathcal K}}
\newcommand{\LLL}{{\mathcal L}}
\newcommand{\MMM}{{\mathcal M}}
\newcommand{\NNN}{{\mathcal N}}
\newcommand{\OOO}{{\mathcal O}}
\newcommand{\PPP}{{\mathcal P}}
\newcommand{\QQQ}{{\mathcal Q}}
\newcommand{\RRR}{{\mathcal R}}
\newcommand{\SSS}{{\mathcal S}}
\newcommand{\TTT}{{\mathcal T}}
\newcommand{\UUU}{{\mathcal U}}
\newcommand{\VVV}{{\mathcal V}}
\newcommand{\WWW}{{\mathcal W}}
\newcommand{\XXX}{{\mathcal X}}
\newcommand{\YYY}{{\mathcal Y}}
\newcommand{\ZZZ}{{\mathcal Z}}
%\renewcommand{\Bbb}{\mathbb}
\newcommand{\AAa}{{\mathbb A}}
\newcommand{\BBb}{{\mathbb B}}
\newcommand{\CCc}{{\mathbb C}}
\newcommand{\DDd}{{\mathbb D}}
\newcommand{\EEe}{{\mathbb E}}
\newcommand{\FFf}{{\mathbb F}}
\newcommand{\GGg}{{\mathbb G}}
\newcommand{\HHh}{{\mathbb H}}
\newcommand{\IIi}{{\mathbb I}}
\newcommand{\JJj}{{\mathbb J}}
\newcommand{\KKk}{{\mathbb K}}
\newcommand{\LLl}{{\mathbb L}}
\newcommand{\MMm}{{\mathbb M}}
\newcommand{\NNn}{{\mathbb N}}
\newcommand{\OOo}{{\mathbb O}}
\newcommand{\PPp}{{\mathbb P}}
\newcommand{\QQq}{{\mathbb Q}}
\newcommand{\RRr}{{\mathbb R}}
\newcommand{\SSs}{{\mathbb S}}
\newcommand{\TTt}{{\mathbb T}}
\newcommand{\UUu}{{\mathbb U}}
\newcommand{\VVv}{{\mathbb V}}
\newcommand{\WWw}{{\mathbb W}}
\newcommand{\XXx}{{\mathbb X}}
\newcommand{\YYy}{{\mathbb Y}}
\newcommand{\ZZz}{{\mathbb Z}}

\newcommand{\OOne}{\mathbbm{1}}
\newcommand{\TTwo}{\mathbbm{2}}
\newcommand{\TThree}{\mathbbm{3}}
\newcommand{\FFour}{\mathbbm{4}}
\newcommand{\FFive}{\mathbbm{5}}
\newcommand{\SSix}{\mathbbm{6}}
\newcommand{\SSeven}{\mathbbm{7}}
\newcommand{\EEight}{\mathbbm{8}}
\newcommand{\NNine}{\mathbbm{9}}

\newcommand{\AaA}{{\mathfrak A}}
\newcommand{\BbB}{{\mathfrak B}}
\newcommand{\CcC}{{\mathfrak C}}
\newcommand{\DdD}{{\mathfrak D}}
\newcommand{\EeE}{{\mathfrak E}}
\newcommand{\FfF}{{\mathfrak F}}
\newcommand{\GgG}{{\mathfrak G}}
\newcommand{\HhH}{{\mathfrak H}}
\newcommand{\IiI}{{\mathfrak I}}
\newcommand{\JjJ}{{\mathfrak J}}
\newcommand{\KkK}{{\mathfrak K}}
\newcommand{\LlL}{{\mathfrak L}}
\newcommand{\MmM}{{\mathfrak M}}
\newcommand{\NnN}{{\mathfrak N}}
\newcommand{\OoO}{{\mathfrak O}}
\newcommand{\PpP}{{\mathfrak P}}
\newcommand{\QqQ}{{\mathfrak Q}}
\newcommand{\RrR}{{\mathfrak R}}
\newcommand{\SsS}{{\mathfrak S}}
\newcommand{\TtT}{{\mathfrak T}}
\newcommand{\UuU}{{\mathfrak U}}
\newcommand{\VvV}{{\mathfrak V}}
\newcommand{\WwW}{{\mathfrak W}}
\newcommand{\XxX}{{\mathfrak X}}
\newcommand{\YyY}{{\mathfrak Y}}
\newcommand{\ZzZ}{{\mathfrak Z}}

\newcommand{\aaA}{{\mathfrak a}}
\newcommand{\bbB}{{\mathfrak b}}
\newcommand{\ccC}{{\mathfrak c}}
\newcommand{\ddD}{{\mathfrak d}}
\newcommand{\eeE}{{\mathfrak e}}
\newcommand{\ffF}{{\mathfrak f}}
\newcommand{\ggG}{{\mathfrak g}}
\newcommand{\hhH}{{\mathfrak h}}
%\newcommand{\IiI}{{\mathfrak I}}
%\newcommand{\JjJ}{{\mathfrak J}}
%\newcommand{\KkK}{{\mathfrak K}}
%\newcommand{\LlL}{{\mathfrak L}}
%\newcommand{\MmM}{{\mathfrak M}}
%\newcommand{\NnN}{{\mathfrak N}}
%\newcommand{\OoO}{{\mathfrak O}}
%\newcommand{\PpP}{{\mathfrak P}}
%\newcommand{\QqQ}{{\mathfrak Q}}
%\newcommand{\RrR}{{\mathfrak R}}
%\newcommand{\SsS}{{\mathfrak S}}
%\newcommand{\TtT}{{\mathfrak T}}
%\newcommand{\UuU}{{\mathfrak U}}
%\newcommand{\VvV}{{\mathfrak V}}
%\newcommand{\WwW}{{\mathfrak W}}
%\newcommand{\XxX}{{\mathfrak X}}
%\newcommand{\YyY}{{\mathfrak Y}}
%\newcommand{\ZzZ}{{\mathfrak Z}}


\newcommand{\mathbold}[1]{\mbox{\boldmath $#1$}}

\newcommand{\aaa}{{\mathbold a}}
\newcommand{\bbb}{{\mathbold b}}
\newcommand{\ccc}{{\mathbold c}}
\newcommand{\ddd}{{\mathbold d}}
\newcommand{\eee}{{\mathbold e}}
\newcommand{\fff}{{\mathbold f}}
\renewcommand{\ggg}{{\mathbold g}}
\newcommand{\hhh}{{\mathbold h}}
\newcommand{\iii}{{\mathbold i}}
\newcommand{\jjj}{{\mathbold j}}
\newcommand{\kkk}{{\mathbold k}}
\newcommand{\elll}{{\mathbold \ell}}
\newcommand{\mmm}{{\mathbold m}}
\newcommand{\nnn}{{\mathbold n}}
\newcommand{\ooo}{{\mathbold o}}
\newcommand{\ppp}{{\mathbold p}}
\newcommand{\qqq}{{\mathbold q}}
\newcommand{\rrr}{{\mathbold r}}
\newcommand{\sss}{{\mathbold s}}
\newcommand{\ttt}{{\mathbold t}}
\newcommand{\uuu}{{\mathbold u}}
\newcommand{\vvv}{{\mathbold v}}
\newcommand{\www}{{\mathbold w}}
\newcommand{\xxx}{{\mathbold x}}
\newcommand{\yyy}{{\mathbold y}}
\newcommand{\zzz}{{\mathbold z}}

\mathcode`\<="4268 %left delimiter
\mathcode`\>="5269 %right delimiter
\mathchardef\gt="313E %relation >
\mathchardef\lt="313C %relation <


%  %===========================================================================
%  %      P. TAYLOR'S "END OF PROOF BOX":
%  %
%  %
%  %  The complexity of the macro necessary to get a little box on the
%  %  right-hand-side at the end of a proof is amazing.  It really does
%  %  have to be this long!  Otherwise you're liable to get it at the
%  %  beginning of the next line, or even on the next page.
%  %
%  \def\pushright#1{{%              set up
%     \parfillskip=0pt            % so \par doesnt push \square to left
%     \widowpenalty=10000         % so we dont break the page before \square
%     \displaywidowpenalty=10000  % ditto
%     \finalhyphendemerits=0      % TeXbook exercise 14.32
%    %
%    %                 horizontal
%     \leavevmode                 % \nobreak means lines not pages
%     \unskip                     % remove previous space or glue
%     \nobreak                    % don't break lines
%     \hfil                       % ragged right if we spill over
%     \penalty50                  % discouragement to do so
%     \hskip.2em                  % ensure some space
%     \null                       % anchor following \hfill
%     \hfill                      % push \square to right
%     {#1}                        % the end-of-proof mark (or whatever)
%    %
%    %                   vertical
%     \par}}                      % build paragraph
% 
%  % prefer proofs with statements, also space after
%  \def\qed{\pushright{$\square$}\penalty-700 \smallskip}

%%=====================================================================
%
%       For laying out a proof:  \begin{prf}{} ... \end{prf}
%       The argument is in case the proof is a continuation as in:
%               \begin{prf}{\ref{four-color} continued} ... \end{prf}
%       if you do not use the argument be careful to use the brackets!
%
%  							due to RAGS
%-----------------------------------------------------------------------

% \newenvironment{prf}[1]{\begin{trivlist} \item[{\it ~Proof}#1.]}%
% {\qed\end{trivlist}}

\newcommand{\be}[1]{\begin{#1}}
\newcommand{\bbe}[2]{\begin{#1}[#2]}
\newcommand{\ee}[1]{\end{#1}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\ba}[1]{\begin{array}{#1}}
\newcommand{\ea}{\end{array}}
\newcommand{\bea}{\begin{eqnarray}}
\newcommand{\eea}{\end{eqnarray}}
\newcommand{\bear}{\begin{eqnarray*}}
\newcommand{\eear}{\end{eqnarray*}}
%\newcommand{\bpr}{\begin{prf}{}}
%\newcommand{\epr}{\end{prf}}
%\newcommand{\bprf}[1]{\begin{prf}{#1}}
%\newcommand{\eprf}{\end{prf}}


\newcommand{\Up}[1]{{\Uparrow}{#1}}
\newcommand{\Do}[1]{{\Downarrow}{#1}}
\newcommand{\UD}[1]{{\Updownarrow}{#1}}
\newcommand{\DoU}[1]{\Do{\Up{#1}}}
\newcommand{\UpD}[1]{\Up{\Do{#1}}}

%\newcommand{\Id}{\mathrm{Id}}


\newcommand{\lft}[1]{\protect\overleftarrow{#1}}
\newcommand{\rgt}[1]{\protect\overrightarrow{#1}}
\newcommand{\Lft}[1]{{\overset{\Longleftarrow}{#1}}}
\newcommand{\Rgt}[1]{{\overset{\Longrightarrow}{#1}}}

\newcommand{\cut}[1]{\protect\overleftrightarrow{#1}} 

%\newcommand{\supp}{\underrightarrow{\rm lim}\ }
%\newcommand{\inff}{\underleftarrow{\rm lim}\ }
%\newcommand{\limsupp}{\protect\overleftarrow{\rm lim}\ }
%\newcommand{\liminff}{\overrightarrow{\rm lim}\ }
\newcommand{\supp}{\mathop{\protect\underrightarrow{\mathrm{lim}}}}
\newcommand{\inff}{\mathop{\protect\underleftarrow{\mathrm{lim}}}}
\newcommand{\limsupp}{\mathop{\protect\overleftarrow{\mathrm{lim}}}}
\newcommand{\liminff}{\mathop{\protect\overrightarrow{\mathrm{lim}}}}

\newcommand{\Dabla}{\curlyvee\hspace{-1.9ex}\curlywedge}
%{\mbox{\begin{sideways} $\bowtie$\end{sideways}}}
\newcommand{\cmnd}[1]{\blacklozenge}%{\Dabla{#1}}
\newcommand{\cmn}{\blacktriangle}%{\curlywedge}%{{\rm \Delta}}
\newcommand{\mnd}{\blacktriangledown}%{\curlyvee}%{\nabla}
\newcommand{\cmnn}[2]{[{#1},\ \Delta {#2}]}
\newcommand{\mndd}[2]{[\nabla {#2},\ {#1}]}
\newcommand{\ccmn}{\curlywedgeuparrow}
\newcommand{\mmnd}{\curlyveedownarrow}

\newcommand{\eh}[1]{\widehat{#1}}%{\{{#1}\}}%{\widehat{#1}}

\newcommand{\tprod}{\textstyle\prod}
\newcommand{\tcoprod}{\textstyle\coprod}
\newcommand{\tint}{\textstyle\int}
\newcommand{\ohm}{{\rm \Omega}}



\newcommand{\Dashv}{\mathrel{\mbox{$={\kern-1.1ex}|$}}}
\renewcommand{\vDash}{\mathrel{\mbox{$|{\kern-1.1ex}=$}}}
\newcommand{\sDashv}{=\!|}
\newcommand{\svDash}{|\!=}

\newcommand{\para}[1]{\medskip\noindent\textbf{#1}}

%\newcommand{\Lfun}[1]{{#1}^\#}
%\newcommand{\Rfun}[1]{{#1}_\#}
%\newcommand{\lan}[1]{{#1}^\ast}
%\newcommand{\ran}[1]{{#1}_\ast}
%\newcommand{\Lan}[1]{{#1}^\circledast}
%\newcommand{\Ran}[1]{{#1}_\circledast}
%\newcommand{\Lmon}[1]{\lft{#1}}
%\newcommand{\Rmon}[1]{\rgt{#1}}
%\newcommand{\LC}{\lan{H}}
%\newcommand{\RC}{\ran{H}}
%\newcommand{\RLC}{{\Rmon{H}}}
%\newcommand{\LRC}{{\Lmon{H}}}
%\newcommand{\St}{{\rm St}}
%\newcommand{\Boo}{{\sf Bool}}
%\newcommand{\Top}{{\sf Top}}
%\newcommand{\Set}{{\sf Set}}

%\newcommand{\mdl}[2]{\left({#1}\vDash {#2}\right)}
%\newcommand{\mdll}[3]{\left({#2}\vDash {#3}\right)_{#1}}

%\newcommand{\closeto}{\leadsto} 
%\newcommand{\biarrow}{\looparrowright}
%\newcommand{\biarrowleft}{\looparrowleft}
%

%\newcommand{\clsr}[1]{\bigl[{#1}\bigr]}
%\newtheorem{conjecture}[theorem]{Conjecture}
%
%		    
%
%\DeclareMathOperator{\Img}{Im}
%\DeclareMathOperator{\Retr}{Retr}
\DeclareMathOperator{\Sub}{{\sf Sub}}
\DeclareMathOperator{\Dfib}{{\sf Dfib}}
\DeclareMathOperator{\Ofib}{{\sf Ofib}}
\DeclareMathOperator{\Con}{{\rm Cones}}
\DeclareMathOperator{\Coc}{{\rm Cocones}}
\DeclareMathOperator{\Arr}{{\sf Arr}}
\DeclareMathOperator{\Lan}{{\rm Lan}}
\DeclareMathOperator{\Ran}{{\rm Ran}}

%\newcommand{\Con}[2]{{\rm Con}_{#1} \left(#2\right)}
%\newcommand{\Coc}[2]{{\rm Coc}_{#1} \left(#2\right)}


%\newcommand{\place}{\mathord{-}}
%\newcommand{\Setaf}[1]{#1\textnormal{-}\Set_{1,\textnormal{free}}}
%\newcommand{\Seta}[1]{#1\textnormal{-}\Set}
%\newcommand{\abs}[1]{\lvert{#1}\rvert}
%\newcommand{\Bool}{\mathbf{B}}
%\newcommand{\PtSet}{\mathsf{PtSet}}
%\newcommand{\Upper}[1]{{\uparrow}{#1}}
%\newcommand{\Lower}[1]{{\downarrow}{#1}}
%%\newcommand{\Upper}[1]{{\Uparrow}_{\{0,1\}}{#1}}
%%\newcommand{\Lower}[1]{{\Downarrow}_{\{0,1\}}{#1}}
%\newcommand{\UpperLower}[1]{{\updownarrow}{#1}}

%\newcommand{\Coms}{G}
%\newcommand{\Mods}{M}
%\newcommand{\coms}{c_\Coms}
%\newcommand{\mods}{c_\Mods}
%\newcommand{\Movs}{R}

%%\newcommand{\Ztwo}{{\ZZz/2\ZZz}}
%\newcommand{\zpz}{{\ZZz_p}}
%%\newcommand{\od}[2]{1\cdot{#1}+(\zpz)\cdot{#2}}
%\newcommand{\od}[2]{\underline{1}{#1}+\underline{p}{#2}}
%\newcommand{\odl}[1]{\underline{1}{#1}}
%\newcommand{\odr}[1]{\underline{p}{#1}}
%\newcommand{\odx}{0}

%\usepackage{mathtools}
%\DeclarePairedDelimiterX{\setcompre}[2]{\{}{\}}{#1\mathrel{}\delimsize|\mathrel{}#2}

\newcommand{\TKL}{\overleftarrow{\KKK}}
\newcommand{\TEM}{\overleftarrow{\EEE}}
\newcommand{\SKL}{\overrightarrow{\KKK}}
\newcommand{\SEM}{\overrightarrow{\EEE}}
\newcommand{\NKL}{\KKK}
\newcommand{\NEM}{\EEE}

\newcommand{\Nat}{{\rm Nat}}
\newcommand{\Niso}{{\rm Iso}}





\newcommand{\Kar}[1]{\underline{#1}}
\newcommand{\Karm}[2]{{#1}_{\overset{\Longleftarrow}%{\looparrowleft}
{#2}}}
\newcommand{\Karc}[2]{{#1}_{\overset{\Longrightarrow}%{\looparrowright}
{#2}}}
\newcommand{\Klm}[2]{{{#1}}_{\protect\overleftarrow{#2}}}
\newcommand{\KlM}[2]{{{#1}}_{\protect\overset{\Leftarrow}{#2}}}
\newcommand{\Klma}[2]{{{\Kar #1}}_{\protect\overleftarrow{#2}}}
\newcommand{\Rlm}[2]{{\widehat{#1}}_{\protect\overleftarrow{#2}}}
\newcommand{\Emm}[2]{{{#1}}^{\protect\overleftarrow{#2}}}
\newcommand{\EmM}[2]{{{#1}}^{\protect\overset{\Leftarrow}
{#2}}}
\newcommand{\Emma}[2]{{\Kar{#1}}^{\protect\overleftarrow{{#2}}}}
\newcommand{\EMM}[2]{\left(\Emc {#1} {#2}\right)^{\overset{\Longleftarrow}{#2}}}
\newcommand{\EMMa}[2]{\left(\Emca {{#1}} {{#2}}\right)^{\overset{\Longleftarrow}{#2}}}
\newcommand{\Klc}[2]{{{#1}}_{\protect\overrightarrow{#2}}}
\newcommand{\KlC}[2]{{{#1}}_{\protect\overset{\Rightarrow}{#2}}}
\newcommand{\Klca}[2]{{{\Kar #1}}_{\protect\overrightarrow{#2}}}
\newcommand{\Rlc}[2]{{\widehat{#1}}_{\protect\overrightarrow{#2}}}
\newcommand{\Emc}[2]{{{#1}}^{\protect\overrightarrow{#2}}}
\newcommand{\EmC}[2]{{{#1}}^{\protect\overset{\Rightarrow}
{#2}}}
\newcommand{\Emca}[2]{{\Kar{#1}}^{\protect\overrightarrow{{#2}}}}
\newcommand{\EMC}[2]{\left(\Emm {#1} {#2}\right)^{\overset{\Longrightarrow}{#2}}}
\newcommand{\EMCa}[2]{\left(\Emma {{#1}} {{#2}}\right)^{\overset{\Longrightarrow}{#2}}}
\newcommand{\Ec}[2]{{\Kar #1}^{\overset{\Longrightarrow}%{\looparrowleft}
{#2}}}
\newcommand{\Em}[2]{{\Kar #1}^{\overset{\Longleftarrow}%{\looparrowright}
{#2}}}

\newcommand{\krgt}[1]{{\overset{\Longrightarrow}{#1}}}
\newcommand{\Karco}[2]{{#1}_{\protect\overrightarrow{#2}}^{\circlearrowleft}}
\newcommand{\Karmo}[2]{{#1}_{\protect\overleftarrow{#2}}^{\circlearrowleft}}
\newcommand{\Karce}[2]{{#1}^{\protect\overrightarrow{#2}}_{\circlearrowleft}}
\newcommand{\Karme}[2]{{#1}^{\protect\overleftarrow{#2}}_{\circlearrowleft}}
\newcommand{\Karmks}[2]{{#1}^{\bullet}_{{#2}}}
\newcommand{\Karcks}[2]{{#1}^{\bullet}_{{#2}}}
\newcommand{\Karmes}[2]{{#1}_{\bullet}^{{#2}}}
\newcommand{\Karces}[2]{{#1}_{\bullet}^{{#2}}}

\newcommand{\ladj}[1]{{#1}^\ast}
\newcommand{\radj}[1]{{#1}_\ast}
%\newcommand{\adj}[1]{\left( \ladj {#1} \dashv \radj {#1}\right)}
\newcommand{\adj}[1]{\ladj {#1} \dashv \radj {#1}}
\newcommand{\lbadj}[1]{{#1}_{!}}
\newcommand{\rbadj}[1]{\ladj{#1}}
\newcommand{\badj}[1]{\lbadj {#1} \dashv \rbadj {#1}}
\newcommand{\upadj}[1]{\begin{minipage}{4mm}$\scriptstyle \ladj {#1}$\\[-1ex]$\scriptstyle \bot$\\[-1ex]$\scriptstyle \radj {#1}$ \end{minipage}}
\newcommand{\lkadj}[1]{{#1}^\flat}
\newcommand{\rkadj}[1]{{#1}_\flat}
%\newcommand{\kadj}[1]{\left(\lkadj{#1} \dashv \rkadj {#1}\right)}
\newcommand{\kadj}[1]{\lkadj{#1} \dashv \rkadj {#1}}
\newcommand{\lnadj}[1]{{#1}^\sharp}
\newcommand{\rnadj}[1]{{#1}_\sharp}
\newcommand{\nadj}[1]{\lnadj{{#1}} \dashv \rnadj {{#1}}}
\newcommand{\lnnadj}[1]{{#1}^{\sharp\sharp}}
\newcommand{\rnnadj}[1]{{#1}_{\sharp\sharp}}
\newcommand{\nnadj}[1]{\lnnadj{{#1}} \dashv \rnnadj {{#1}}}
\newcommand{\loadj}[1]{{#1}^\natural}
\newcommand{\roadj}[1]{{#1}_\natural}
\newcommand{\oadj}[1]{\loadj{{#1}} \dashv \roadj {{#1}}}
\newcommand{\lpadj}[1]{{#1}^\bullet}
\newcommand{\rpadj}[1]{{#1}_\bullet}
\newcommand{\padj}[1]{\lpadj{{#1}} \dashv \rpadj {{#1}}}
\newcommand{\liadj}[1]{\overline{#1}^\ast}
\newcommand{\riadj}[1]{\overline{#1}_\ast}
\newcommand{\iadj}[1]{\left(\liadj{{#1}} \dashv \riadj {{#1}}\right)}


\newcommand{\ladja}[1]{{\Kar{#1}}^\ast}
\newcommand{\radja}[1]{{\Kar{#1}}_\ast}
\newcommand{\adja}[1]{\ladj {\Kar{#1}} \dashv \radj {\Kar{#1}}}
\newcommand{\upadja}[1]{\begin{minipage}{4mm}$\scriptstyle \ladja{#1}$\\[-1ex]$\scriptstyle \bot$\\[-1ex]$\scriptstyle \radja{#1}$ \end{minipage}}
\newcommand{\lkadja}[1]{{\Kar{#1}}^\flat}
\newcommand{\rkadja}[1]{{\Kar{#1}}_\flat}
\newcommand{\kadja}[1]{\lkadja{#1} \dashv \rkadja{#1}}
\newcommand{\lnadja}[1]{{\Kar{#1}}^\sharp}
\newcommand{\rnadja}[1]{{\Kar{#1}}_\sharp}
\newcommand{\nadja}[1]{\lnadja{{#1}} \dashv \rnadja {{#1}}}
\newcommand{\lnnadja}[1]{{\Kar{#1}}^{\sharp\sharp}}
\newcommand{\rnnadja}[1]{{\Kar{#1}}_{\sharp\sharp}}
\newcommand{\nnadja}[1]{\lnnadj{{#1}} \dashv \rnnadj {{#1}}}
\newcommand{\loadja}[1]{{\Kar{#1}}^\natural}
\newcommand{\roadja}[1]{{\Kar{#1}}_\natural}
\newcommand{\oadja}[1]{\loadja{{#1}} \dashv \roadja{{#1}}}
\newcommand{\lpadja}[1]{{\Kar{#1}}^\bullet}
\newcommand{\rpadja}[1]{{\Kar{#1}}_\bullet}
\newcommand{\padja}[1]{\lpadja{{#1}} \dashv \rpadja{{#1}}}
\newcommand{\liadja}[1]{\overline{\Kar{#1}}^\ast}
\newcommand{\riadja}[1]{\overline{\Kar{#1}}_\ast}
\newcommand{\iadja}[1]{\left(\liadja{{#1}} \dashv \riadja {{#1}}\right)}


%\newcommand{\CM}[1]{\CCC\left({#1}\right)}
%\newcommand{\MN}[1]{\MMM\left({#1}\right)}
%
%\newcommand{\subl}[2]{_{{#1}}{{#2}}}
%\newcommand{\supl}[2]{^{{#1}}{{#2}}}
%\newcommand{\compson}{K}

%\newcommand{\NEM}{\EEE}

\newcommand{\co}[1]{\overline{#1}}

\newcommand{\OObj}{{\cal J}}
\newcommand{\AAtr}{{\cal U}}
\newcommand{\Obj}{{\sf J}}
\newcommand{\Atr}{{\sf U}}
\newcommand{\Rat}{{\sf R}}
\newcommand{\Tr}{{\rm tr}}
\newcommand{\Prob}{{\rm P}}
\newcommand{\Sim}{{\rm s}}
\newcommand{\SSim}{{\rm s}}
\newcommand{\Dist}{{\rm d}}
\newcommand{\Exp}{{\bf E}}
%\newcommand{\bal}[1]{{#1}^0}

\newcommand{\Ess}{{\sf Ess}}
\newcommand{\Ffa}{{\sf Ffa}}

\newcommand{\compson}{H}
\newcommand{\compss}{\Xi}
\newcommand{\compstwo}{K}
\newcommand{\compskl}{E}

 \newcommand{\cuu}[1]{\Lbag{#1}\Rbag} 
 
 \newcommand{\retr}{\begin{tikzar}[column sep = 1.3em]
\hspace{.1ex} \ar[thin,tail,bend right=15]{r} \& \hspace{.1ex} \ar[thin,two heads,bend right=15]{l}\end{tikzar}
}  

\newcommand{\restr}{\!\!\restriction}
\newcommand{\Pow}{\PPP}

\hyphenation{mo-no-idal}%,Gro-then-dieck}
%\babelhyphenation[english]{every-where}


